Efficient Domain Adaptation via Generative Prior for 3D Infant Pose Estimation

Although 3D human pose estimation has gained impressive development in recent years, only a few works focus on infants, that have different bone lengths and also have limited data. Directly applying adult pose estimation models typically achieves low performance in the infant domain and suffers from out-of-distribution issues. Moreover, the limitation of infant pose data collection also heavily constrains the efficiency of learning-based models to lift 2D poses to 3D. To deal with the issues of small datasets, domain adaptation and data augmentation are commonly used techniques. Following this paradigm, we take advantage of an optimization-based method that utilizes generative priors to predict 3D infant keypoints from 2D keypoints without the need of large training data. We further apply a guided diffusion model to domain adapt 3D adult pose to infant pose to supplement small datasets. Besides, we also prove that our method, ZeDO-i, could attain efficient domain adaptation, even if only a small number of data is given. Quantitatively, we claim that our model attains state-of-the-art MPJPE performance of 43.6 mm on the SyRIP dataset and 21.2 mm on the MINI-RGBD dataset.

==> sec/01_abs.tex <==
\begin{abstract}
Although 3D human pose estimation has gained impressive development in recent years, only a few works focus on the infants, which has different bone lengths and also has limited data. Directly applying adult pose estimation models typically achieves low performance in the infant domain and suffers from out-of-distribution issues. Moreover, the limitation of infant pose data also heavily constrains the efficiency of learning-based models to lift 2D poses to 3D. For small datasets, domain adaptation, and data augmentation are commonly used techniques. Following this paradigm, we take advantage of an optimization-based method that utilizes generative priors to predict 3D infant keypoints from 2D keypoints.  We further applied a guided diffusion model converting 3D adult pose to infant pose to supplement small datasets.  Besides, we also prove that our method, InfPose, could attain efficient domain adaptation, even if only a small number of data is given, to simulate the extreme condition when data is limited. Quantitatively, we claim that our model attains state-of-the-art MPJPE performance of \textbf{43.6} mm on the SyRIP dataset which is \textbf{34.9} mm better than previous SOTA and \textbf{21.2} mm on the MINI-RGBD dataset, that is \textbf{7.3} mm less than the previous SOTA.
\end{abstract}

==> sec/02_intro.tex <==
\section{Introduction}
3D human pose estimation is always a popular area these days. Similarly, pose estimation for infants plays an important role in risk assessment and healthcare monitoring\cite{Pierratn741}. However, due to privacy and the difficulty of data collection, public infant pose datasets are rare and limited, and manual labeling is unreliable and expensive. Therefore, it is challenging to train an efficient deep-learning model from scratch without sufficient data. To address this limitation, it is natural to think about transferring or tuning an existing adult-based pose estimation model on infant datasets to fully take advantage of similar kinetics of human body pose. Previous work like \cite{syrip} tried to adapt a 2D adult pose detector to the infant domain, but little work has been discussed in terms of 3D infant pose estimation. So in this paper, we would like to pursue a method that can efficiently predict 3D infant poses even in small infant datasets, with the general kinetic knowledge transferred from adult based pre-trained model, as the outline shown in figure \ref{fig:big_pic}.
\begin{figure}[t]
\centering
  \includegraphics[width=\linewidth]{figure/old_outline.png}
  \caption{The overall outline of our method. Our model aims to adapt a generative prior pre-trained on large adult pose data to the infant domain via a controllable branch. Then, we utilize generative prior in the infant domain to do optimization work that predicts 3D infant pose from 2D pose.}
  \label{fig:big_pic}
\end{figure}


Though learning-based 3D pose estimation models typically learn better features and obtain higher performance compare to optimization algorithms, they apparently require much more data in training for sufficient feature learning. Besides, the majority of  human pose estimation learning models suffer from out-of-distribution issues which makes them hard to apply in practical scenarios or datasets which are far from the training data. However, this can easily happen for infant pose as few public datasets are available to support a more general 3D model's training, and cameras in hospitals or healthcare institutions may have different camera settings, leading to an unpredictable domain gap. Fortunately, previous optimization works \cite{bogo2016smplify, thomas2018joint} are proved to be more insusceptible to distribution bias and robust in cross-domain tasks. Moreover, thanks to sophisticated 2D keypoint detectors, two-stage lifting networks are generally of higher accuracy than one-stage networks which directly predict 3D pose from raw images. In addition, we believe that generative models can be easily trained with few data and be domain-adapted efficiently compared to classic deep-learning models. Therefore, inspired by ZeDO\cite{jiang2023back}, we choose to apply a two-stage optimization-based method named IZeDO to address lack of data and out-of-distribution issues, under the assistance of generative priors. Given 2D keypoints, our model can iteratively adjust noisy 3D prediction under the constraint of 2D-3D projection and prior distribution learned. As we expected, generative priors learned in the adult domain could be easily transferred to the infant domain without requiring much data, and the optimization process can cope with challenging test data in reality. Moreover, to simulate the extreme condition of lack of data in small datasets, we also test our model with only 20 and 100 data during adaption and successfully validate our model's capacity of efficient domain adaptation. Furthermore, we also introduce a guided diffusion model which aims to supplement datasets by converting adult pose to infant pose, in order to address data limitation issues and reinforcement diversity. Finally, our method obtain SOTA performance in terms of MPJPE (Mean Per Joint Position Error) on two infant pose datasets. 
In this paper, we make the following contributions: 
% \\
% % 1. We proposed a new architecture to adapt a diffusion model trained on adult pose keypoints to meet infant kinetics without polluting the original network. Taking this domain-adapted diffusion model as backbone, out model's performance is comparable to direct fine-tuning and even better in a challenging dataset SyRIP ~\cite{} which is more close to practical scenarios. 
% \\

\begin{itemize}
    \item We propose an optimization based method using generative priors for 3D infant pose estimation. We attain SOTA performance on MINI-RGBD\cite{mini} and SyRIP\cite{syrip}. We also claim that our model can do efficient domain-adaptation even with a small number of data.
   
    \item We introduced a condition-guided diffusion model which can convert adult human keypoints to similar infant keypoints for data augmentation purpose, and further enhance performance.
\end{itemize}


==> sec/03_related_works_new.tex <==
\section{Related Work}

\subsection{3D Human Pose Estimation}
3D Human Pose Estimation is one of the fundamental tasks in computer vision and is crucial to many downstream tasks including Human Tracking\cite{andriluka2018posetrack, wang2020combining}, Action Recognition\cite{zhou2021hierarchical, yang2022unsupervised, duan2022revisiting}, Motion Analysis\cite{howe1999bayesian, jiang2022golfpose}, and so on. There are three main tracks in the 3D human pose estimation area: optimization-based, 2D-3D lifting, and image-based methods. Optimization-based methods are not limited by any training datasets and are good at in-the-wild inference. However, the performance of previous optimization-based methods\cite{bogo2016smplify, tang2018joint, muller2021SMPLify-XMC} is worse than the performance of training-based networks. 

2D-3D lifting methods follow a two-stage pipeline requiring a separate 2D human pose estimation model and take advantage of learning to map 2D human poses to 3D human poses in single frames or short sequences. Pavllo \etal~\cite{pavllo20193d} apply dilated temporal convolution to enhance 3D pose estimation for unlabeled videos in a semi-supervised method. Zhao \etal~\cite{zhao2019semantic} designs a novel graph convolution and takes advantage of GCN to learn inter-joint features and local and global relationships in a structured graph. On the other hand, image-based methods focus on directly regressing 3D human poses from RGB images. Kolotouros \etal~\cite{kolotouros2019learning} propose SPIN by using a CNN to extract features from a cropped-out human image and regress the SMPL~\cite{SMPL} parameters with the help of an optimization-based pose estimation pipeline to conduct semi-supervised learning. VIBE~\cite{kocabas2019vibe}, proposed by Kocabas \etal, utilizes additional temporal information and achieves better performance. However, all the learning-based methods suffer from small datasets in Infant Pose Estimation tasks. In this paper, we focus on how to conduct 3D infant pose estimation with limited data.
% Optimization method is good at doing inference case by case and not easily influenced by domain gap and out-of-distribution issue. SMPLify\cite{bogo2016smplify} uses SMPL\cite{SMPL} model to do optimization via minimizing kinetic constraints and model to 2D projection error. Furthermore, SMPLift-XMC\cite{muller2021SMPLify-XMC} takes into account of age and height, and add more advanced constraints on the base of SMPLify. In \cite{8486576}, they build a novel video scene system to predict 3D pose, tracklets and actions under overlapping views collected by cameras. In \cite{wang2014robust}, they represent a 3D pose as a linear combination of base learned from 3D skeletons and also follow 3D-2D projection constraints and limb length. Optimization work does not depend on the number of data much for training but requires high accuracy of 2D detection. In the case of small datasets, we believe that an optimization track is more reliable than learning-based models.

% \subsection{2D-3D Lifting Network in Human Pose Estimation}
% There are mainly two tracks in the human pose estimation area. One-stage method aim to direclty predict 3D keypoints or model from raw images, and two-stage ones use 2D  detector to extract 2D keypoints first as an intermediate step and lift 2D to 3D. For instance, 
% In \cite{pavllo20193d}, they apply dilated temporal convolution to enhance 3D pose estimation for unlabeled videos in an semi-supervised method. Zhao \etal\cite{zhao2019semantic} designs a novel graph convolution and takes advantage of GCN to learn inter-joint features and local and global relationships in a structured graph.  Yang \etal \cite{yang2023camerapose} choose to use the 2D annotations in the wild to improve prediction quality, in an weakly supervised method.
% Traditionally, one-stage method is more challenging as images may vary to a great extent so it is generally harder to do inference in the wild or cross evaluation. Therefore we follow two-stage track for accuracy as 2D detectors now are fully developed, even in the infant domain\cite{syrip}.

% \subsection{Diffusion Model in Human Pose Estimation}
% Nowadays, diffusion model becomes one of the most popular topics due to its outstanding capacity of image generation and denoising. As a strong generative model, a lot of previous work have proven that it is a reliable prior learner\cite{}. In human pose estimation, ~\cite{} applies a GNN-based backbone and a sequence of 2D pose as conditions to predict 3D keypoints. Furthermore, ~\cite{} uses 2D as condition and proposes a new mask strategy to unify denoising, 3D generation and 3D prediction. Though we choose to apply a Score Matching NetWork diffusion model as our generative priors, our model is only trained on 3D pose data without 2D conditions for guidance. Once 2D condition involves in training, the diffusion model may still suffer from out-of-distribution issues. 

\subsection{Infant Pose Estimation}
% 1) 2D Infant Pose Estimation
% 2) 3D Infant Pose Estimation
% 3) Limitation of existing works
Infant pose estimation aims at predicting 2D and 3D keypoints in image and world coordinates which can lead to useful downstream tasks such as infant action recognition \cite{yang2022unsupervised, huang2023posture} or motion analysis \cite{chambers2020computer, huang2023sym}. Hesse \etal\cite{mini} are the first to present MINI-RGBD dataset which enables the experiment on 2D infant pose estimation followed by Huang \etal\cite{syrip} proposing a hybrid synthetic and real infant pose (SyRIP) dataset based on SMIL \cite{ma2021smil} with annotated 2D keypoints. Following the 2D infant pose estimation, the mainstream of 3D infant pose estimation works on RGB-D data. Wu \etal\cite{wu93} measured infant movements by combining 2D keypoints and matching depth images collected by Kinect. Li~\cite{li2020three} continues using the same pipeline but correcting depth information for a better matching between image and depth. However, Kinect may cause depth ambiguity if joints are occluded, and depth images are not always available in the infant monitor system. In ~\cite{ellershaw3d}, the author uses a 2D pose estimation model and a 3D lifting network pretrained on the adult dataset and fine-tuned on the infant dataset. Though their model achieves rather good performance on the MINI-RGBD dataset, their model is basically learning-based and hard to adapt to more realistic data due to the domain gap. From our experience in human pose estimation, predicting 3D keypoints from 2D keypoint detection is easier than the one-stage method predicting 3D joints from raw images.

==> sec/04_method.tex <==
\section{Methods}

In the following sections, we will introduce our model in such order: background of diffusion model in section~\ref{sec:method_diffusion}, generative prior model in section~\ref{sec:prior model}, optimization algorithm in~\ref{sec:opt}, its controllable adaptation variant in~\ref{sec:ctrl} and condition-guided data augmentation in~\ref{sec:aug}.  

\begin{figure*}[h!]
\centering
  \includegraphics[width=0.95\textwidth]{figure/mod.pdf}
  \caption{\textbf{Model architecture}. The modules excluded by the dotted box are our proposed score-matching-based prior learning model, and the modules inside the dotted box are the controllable branch used in one of our adaptation strategies. The prior learning model consists of MLP layers for input and output projection and two residual blocks. The controllable branch takes a learning prompt as inputs, copies the weights from the prior model and only updates the copied weights during adaptation, while the original prior learning model is kept frozen. For convenience, we paint all frozen layers in controllable adaptation as blue and all updated layers as brown.}
  \label{fig:arch}
\end{figure*}

\subsection{Preliminaries of Diffusion Model}
\label{sec:method_diffusion}
Before introducing our diffusion model as the generative prior learning model, we briefly discuss its background for clarity. Diffusion models~\cite{ho2020denoising,song2020score} are popular generation models used in tasks like image generation~\cite{ramesh2021zero}, image inpainting~\cite{lugmayr2022repaint}, editing~\cite{cao2023difffashion}and so on. During training, diffusion model iteratively add Gaussian noise relative to a timestamp $t$ to the inputs and tries to recover inputs in the reverse process. In this paper, we use Score-Matching-Network(SMN)~\cite{song2020score} as our prior learner. SMN aims to train a score network $s_{\theta}(x)$ to approximate gradients of log probability of a score function $p_{\theta}(x)$, expressed as $s_{\theta}(x) \approx \triangledown_{x} \log{p_{\theta}(x)}$, so the loss is generally represented as 

\begin{equation}
    E_{p(x)} \| \triangledown_{x} \log{p_{\theta}(x)} -  s_{\theta}(x)\|^{2}_2.
\end{equation}

\subsection{Infant Pose Prior Model}
\label{sec:prior model}
For pose estimation tasks on small datasets, learning based deep-learning models suffer from out-of-distribution issues and insufficient resources to capture reliable features. We proposed to use an optimization-based method to predict 3D keypoints from 2D keypoints along with a score-matching network diffusion model(SMN)~\cite{song2020score} as our prior learner, similar to ZeDO~~\cite{jiang2023back}. Our final architecture is displayed in \ref{fig:arch}. The model excluded by the bounding box is our proposed prior learning model which takes root-relative infant keypoints sized $B \times J \times 3$ and randomly sampled noise timestamp $t$ as inputs, where $J$ is the number of joints. The embedding layers are simple linear projection layers which lift input dimension to $B \times 1024$, and then sum them up. Further the embedding goes through the Score-Matching-Network diffusion model consisting of two residual blocks as backbones. For each of the residual block, it contains two residual-connected MLP and GroupNorm layers. The last output projection layer upsamples the feature back to pose joints. With the generative priors, our method can denoise a noisy 3D pose in the optimization stage if it breaks kinematic rules of infant poses.



\subsection{Optimization Work}
\label{sec:opt}
Given a 2D infant pose and the intrinsic parameter, our method first tries to represent the rays emitted by the camera. Supposedly, all these rays go through their corresponding root-relative 3D keypoints which has a 2D projection exactly equal to the 2D pose. In general, our method would keep all the predicted 3D keypoints on the rays and let the generation model adjust the noisy 3D pose prediction based on its prior knowledge. After each adjustment, 3D keypoints may not stay on the rays and we again move them to the rays in the shortest distance to minimize 3D-2D projection error. Our method runs this iteration 1000 times to iteratively achieve a reasonable 3D pose under a 3D-2D projection constraint. 
In experiments, we find that a pseudo intrinsic parameter also functions so one could apply it in the practical cases.
% For convenience, we have our pseudo algorithm summarized in algorithm \ref{alg:pipeline}.
\\
We first compute ray vectors $K^{-1} \dot X_{2D}$ emitted from the camera using real or pseudo intrinsic parameter $K$ and 2D keypoints $X_{2D}$. Then we initialize the initial pose on the rays with an appropriate depth $T_{o}$, and supposedly this 3D initial pose $X_{3D}$ has zero projection error with the 2D pose. Therefore we first randomly choose a training 3D pose $X_{3D_init}$ and use an Adam optimizer~~\cite{kingma2014adam} which helps us find an appropriate rotation $R_{o}$ and translation $T_{o}$ such that $ \|K(R_{o}X_{3D_init} + T_{o}) - X_{2d}\|_2$ is minimized. With $T_{o}$ known, we set all initial 3D keypoints on the rays with depth equal to $T_{o}$. Next, we start $T=1000$ times of optimization in which we first move 3D kyepoints to corresponding rays in the shortest distance if they are off the rays and then let the prior model adjust the noisy pose. 
\\
In evaluation, we find that a noise level $t=(0,0.1]$ works the best. In addition, we find that performance is heavily dependent on initial depth distance assigned. As the training data are all root-relative, the prior model has little knowledge of the absolute depth in space, which means that depth ambiguity may happen if we don't limit depth in the process. In practice, we get the lowest error when forcing the depth equal to the initial depth in the first 950 iterations and open the constraint in the rest 50.  

% To predict 3D keypoints from 2D keypoints and address the one-to-many mapping issues, ZeDO~~\cite{} takes a diffusion model to learn 3D pose prior to denoise a 3D noisy human pose guess from 2D keypoints and meanwhile minimize 3D-2D projection error. The model would first introduce a initial pose to infer translation $T$ and rotation matrix $R$ such that. Then it would do a number of iterations of optimization work given camera parameter. If 2D keypoints and camera parameters are known, one could know the rays emitted from the camera and supposedly all 3D keypoints stay on the rays. At each iteration, all 3D keypoints predicted have to move to the corresponding rays in the shortest distance to minimize projection errors to 2D keypoints. However, these keypoints may not lead to a reasonable human pose so the diffusion backbone would adjust the noisy poses to meet the prior distribution it learns. We continue using the same model as optimization method could effectively avoid out-of-distribution scenarios and easily adopted in different datasets. 

% \subsection{Domain Adaptation of Diffusion Model}
% As adult pose datasets have a much larger number of data as opposed to deprived infant datasets, directly finetuning such model to a small dataset may cause overfitting. Therefore, inspired by Control-Net~~\cite{}, we apply a domain-adaptation structure as shown in to transfer diffusion model pre-trained in adult pose to infant pose domain. 
% \\
% During training, the diffusion backbone pre-trained on adult data keeps frozen and we copied its parameters to the tuning branch. The tuning branch takes a $3*17$ learnable token as condition prompt sums up with noisy input poses, and updates all the parameters on the tuning branch in training. After every layer, the tuning branch will join back to the frozen diffusion model along a zero-initialized convolution layers. 
% \begin{algorithm}[t]
% \caption{InfPose pipeline}\label{alg:pipeline}
% \begin{algorithmic}
% \Require $\text{Initial 3D pose}~X_{init3D}, \text{Target 2D pose}~x_{2D},$ \\ $\text{Pseudo or Camera intrinsic}~K,$ \\ $\text{Diffusion noise level timestamp}~t$,\\ $\text{Pre-trained generative prior model}~\theta_{g}$
% \\

% \State \textcolor{Green}{// \textit{Optimization of inital R and T}}
% \State $V_{ray} = K^{-1}x_{2D}$
% \State $\hat{V_{ray}} = \frac{V_{ray}}{\|V_{ray}\|_2}$
% \State $R_{o}, T_{o} = \min \argmin_{R_{o},T_{o}} \|K(R_{o}X_{init3D} + T_{o}) - x_{2D}\|_2$
% \State \textcolor{gray}{// \textit{Initial Pose}}
% \State $X_{0} = \hat{V_{ray}}*T{o}$
% \State $X_{0} = R_{o}X_{0}$
% \State \textcolor{gray}{// \textit{Iterative Optimization and Denoising}}
% % \State $r \gets K^{-1}p_{2d}$
% % \State $\hat{r} \gets \frac{r}{\|r\|_2}$
% \For{$i = 0$ to $n-1$}
%     \If{$i < depth warmup$}
%         \State $T_i = T_{o}$
%     \Else
%         \State $T_{i} = \min \argmin_{T_i} \|C_{2d}(K(X_{i} + T_{i}) - x_{2d})\|_2$
%     \EndIf
%     \State \textcolor{gray}{// \textit{Move 3D keypoints to rays by projection}}
%     \State $\widetilde{X}_{i} = \Big((X_{i} + T_{i}) \cdot \hat{V_{ray}}\Big)\hat{V_ray} - T_i$
%     \State \textcolor{gray}{// \textit{Adjustment by generative prior}}
%     \State $X_{i+1} = \theta_g(\widetilde{X}_{i}, t(i))$
% \EndFor
% \State return $X_n$
% \end{algorithmic}
% \end{algorithm}


\subsection{Controlling Branch for Domain Adaptation}
\label{sec:ctrl}
As kinematics of infant and adults are similar and adults have more pose data with high diversity, transferring a pre-trained adult pose model to the infant domain would intuitively boost the performance. Considering that directly fine-tuning a model trained on a huge amount of data to a small dataset may lead to overfitting, we propose a method inspired by Control-Net to manipulate the adaption process of the generative priors. Shown in the left side dotted box in figure \ref{fig:arch},  we duplicate the weights of the Score-Matching Network prior model to the controllable branch. We set a $3*17$ sized learnale prompt as controlling inputs, and connect the prior model and controllable branch with a few zero linear layers which are fully initialized as zero weights. To fully integrate controllable branch information with the prior learned in the adult domain, internal embeddings are  added back to the prior model before and after every residual block. During adaptation, all layers of the prior model have to keep frozen and only the controllable branch is open to weight update. In the experiment section, we will compare its performance with two other adaption strategies: fine-tuning a pre-trained adult prior model and training a prior model in infant domain only. 

\subsection{Condition Guided Diffusion Model}
\label{sec:aug}
If the only available data are too few to be used, one could convert the resourceful adult pose to infant-alike poses. To smooth this conversion and also fit the augmented data to the kinematics of infants, we trained a diffusion model which takes both adult and infant poses along with a learnable condition token representing if the pose belongs to adults or infants. We hope that the diffusion model would implicitly learn features like bone lengths and bone angles for two different domains and know how to distinguish their distribution. During inference, we ask the diffusion model to generate corresponding infant poses based on adult poses given, so the model adjusts the scale and angle according to the implicit knowledge of pose prior, yet still keeps the pose semantic meanings like actions, as shown in \ref{fig:augvis}. Though some actions are infeasible for infants, we prove that adding these challenging poses enhance diversity in the ablation study.



\begin{figure}[h!]
\centering
  \includegraphics[width=0.35\textwidth,scale=0.5]{figure/data_aug_vis.jpg}
  \caption{Left: augmented infant pose. Right: h36m adult pose. Our augmentation model converts the adult pose to a similar infant pose by adjusting scales and kinematic features like bone length without altering actions much. }
  \label{fig:augvis}
\end{figure}

==> sec/05_exp.tex <==
\section{Experiments}

\subsection{Datasets}
We launch our experiments on MINI-RGBD\cite{mini} and SyRIP\cite{syrip}, two public infant datasets with 2D-3D pose pairs.

\noindent\textbf{MINI-RGBD} includes 12 sequences of data, in total 12000 synthetic infant images and also provides their 25 joint 2D and 3D keypoint pairs. We train on the first 9 datasets, and test on the rest 3 with 17 keypoints, following the keypoint definition of Human3.6m~\cite{H36M}



\noindent\textbf{SyRIP} includes a diverse set of 700 real and 1000 synthetic infant images generated by fitting SMIL~\cite{ma2021smil} models to real images and adding additional variants to the parameters. Later, they published in total 700 weak ground truth of 3D keypoints in ~\cite{huang2023sym} by manually correcting their predictions. In this paper, we also train on their 600 weak ground truth 3D labels and test on the 100 real images.

\subsection{Implementation Details}
We pre-train our adult generative prior model on Human3.6m\cite{H36M} which includes millions of adult 3D pose data, and train all three adaptation strategies for 5000 epochs with a learning rate of $2\times10^{-4}$. During training, we set the total diffusion step as $1000$ with a uniform noise level of $\left[0, 1.0\right]$. We use the Adam Optimizer with a batch size of $5000$. 


In inference, we choose a noise level $t$ in $\left(0,0.1\right]$ and run the optimization for 1000 iterations. We keep the depth distance unchanged in the first 950 iterations.

The guided diffusion data augmentation diffusion model shares the same training configuration as the prior model. We choose a noise level in the range $\left(0,1.0\right]$ and only run $100$ iterations for the diversity of augmented data. In experiements, we add 600 augmented data to SyRIP and 4000 to MINI-RGBD.


\section{Experiment Results}
In this section, we first compare our method's results to previous SOTA in terms of MPJPE. In addition, we also test if our method can be efficiently adapted to infant domain with 20 and 100 data only in order to simulate extreme situations.  Further, we evaluate all strategies of our model including the controllable adaptation method~(CA), fine-tuning from the adult-based diffusion model~(FT), and training from scratch on infant data to seek the best adaptation approach.


\begin{table}[t]
\centering
\resizebox{0.6\linewidth}{!}{%
\setlength{\tabcolsep}{0.1cm}
\begin{tabular}{l | c }
\toprule
 Methods  & MPJPE~($\downarrow$)\\
\midrule
  Kolotouros~\etal~\cite{kolotouros2019learning} & 105.8 \\
  Liu~\etal~\cite{liu2021heuristic} &  97.2\\
  Liu~\etal(Finetuned)  & 78.3  \\
\midrule
  Our method & \textbf{43.6} \\
 
  % & Ci \etal\cite{ci2023gfpose}~(S=200)(S=200) & 35.6 & 16.9\\

\bottomrule
\end{tabular}
}
\caption{3D infant pose estimation results on SyRIP datast under 12 joints setting. We list the best performance among the three training strategies for different numbers of data $S$ used. The results of other methods are provided by~\cite{huang2023sym} }
\label{tab:syrip}
% \end{adjustbox}
\end{table}

\subsection{Results on SyRIP}
Similar to previous work, we have the same training and testing sets as~\cite{ellershaw3d} and also kept only 12 keypoints of limbs for fair comparison. Observed from Table~\ref{tab:syrip}, our method clearly outperforms the SOTA even with only 20 data. Moreover, as shown in \ref{tab:few_data_syrip}, we observe that fine-tuning and controllable adaptation approaches achieve comparable results, but both better than training from scratch, indicating that knowledge from the adult domain is useful.
% the controllable-adaptation approach achieves comparable results and even lower error when data number is small, demonstrating a better learning capacity for data in reality like SyRIP.


\begin{table}[t]
\centering
\resizebox{0.6\linewidth}{!}{%
\setlength{\tabcolsep}{0.08cm}
\begin{tabular}{l | c }
\toprule
 Methods  & MPJPE~($\downarrow$)\\
\midrule
  Hesse \etal\cite{hesse} & 44.9 \\
  Ellershaw$^*$~\etal\cite{ellershaw3d} &  34.2\\
  Ellershaw~\etal  &  28.5\\
  \midrule
  Our method &  \textbf{21.2}\\
 
  % & Ci \etal\cite{ci2023gfpose}~(S=200)(S=200) & 35.6 & 16.9\\

\bottomrule
\end{tabular}
}
\caption{3D infant pose estimation results on MINI-RGBD under 16 joints setting. We list the best performance among the three strategies. $^*$ denotes w/o adult pre-training. We evaluate on 16 keypoints to keep aligned with the setting of the previous SOTA.}
\label{tab:mini}
% \end{adjustbox}
\end{table}


\subsection{Results on MINI-RGBD}
For fair comparison with previous work, we follow their keypoint definitions and show the results  in table \ref{tab:mini}, our method beats all previous performance to a great extent.
\\
Besides, we find in table \ref{tab:few_data_mini} that direct fine-tuning adult pre-trained model on MINI-RGBD attains lower error, which is different from SyRIP. We suspect that the similarity between training and testing sets leads to this observation, as MINI-RGBD is full of synthetic images with rather low diversity compared to the SyRIP dataset.






==> sec/06_ablation.tex <==
\section{Ablation Studies}

\begin{figure*}[t]
\centering
  \includegraphics[scale = 0.28]{figure/diffusion.jpg}
  \caption{Visualization of the optimization algorithm. $\hat{V_{ray}}$ ray vectors are first calculated.  $T_{o}$ and $R_{o}$ are then found via an optimizer, so the initial pose is $T_{o}$ in depth on the rays. We then run the optimization algorithm 1000 times. In each step, keypoints are moved to the rays, represented by $\tilde{X_{o}}$ in the figure, and are also sent to the diffusion model to adjust the pose to get $X_{0}$. In the last step $X_{1000}$ the ground truth in blue is quite close to our prediction in red.}
  \label{fig:diff}
\end{figure*}

\begin{table}[t]
\centering
\resizebox{0.6\linewidth}{!}{%
\setlength{\tabcolsep}{0.1cm}
\begin{tabular}{l | c | c | c}
\toprule
 Datasets   & CA & FT & From Scratch\\
\midrule
  SyRIP~($S$=20) & \textbf{67.8} &69.4 & 72.3\\
  SyRIP~($S$=100) & \textbf{56.4} & 60.8 & 60.6 \\
  SyRIP   &49.4 & \textbf{47.7} & 54.0\\
  SyRIP~(augmented)   & 45.5 & \textbf{43.6} &48.9\\
 
  
  % & Ci \etal\cite{ci2023gfpose}~(S=200)(S=200) & 35.6 & 16.9\\

\bottomrule
\end{tabular}
}
\caption{MPJPE performance of different strategies on SyRIP. Controllable adaptation approach achieves better performance than the other two.}
\label{tab:few_data_syrip}
% \end{adjustbox}
\end{table}


\begin{figure}[h!]
\centering
  \includegraphics[scale = 0.25]{figure/mini_dis.jpg}
  \caption{Left side: Data distribution of 3D pose of MINI-RGBD Dataset. Right side: Data distribution of the augmentation data for MINI-RGBD. The augmentation data increases diversity.}
  \label{fig:dist_aug}
\end{figure}

\begin{table}[t]
\centering
\resizebox{0.6\linewidth}{!}{%
\setlength{\tabcolsep}{0.1cm}
\begin{tabular}{l | c | c | c| c}
\toprule
 Datasets   & CA & FT & From Scratch & Best\\
\midrule
  MINI-RGBD~($S$=20) & 38.7 & 36.8 & \textbf{36.4} & 34.6\\
  MINI-RGBD~($S$=100) & 34.8 & \textbf{31.9} & 33.7 & 29.4\\
  MINI-RGBD & 25.5 & \textbf{24.1} &27.4 & 22.8\\
  MINI-RGBD~(augmented)  &20.7 &\textbf{19.9} &21.3 & 21.2\\
 
  
  % & Ci \etal\cite{ci2023gfpose}~(S=200)(S=200) & 35.6 & 16.9\\

\bottomrule
\end{tabular}
}
\caption{MPJPE performance of different strategies on MINI-RGBD. Here we evaluate all 17 keypoints as H36M's keypoint definition, but also list their performance in 16 keypoints for convenience of comparison with previous works.}
\label{tab:few_data_mini}
% \end{adjustbox}
\end{table}

% \begin{figure}[h!]
% \centering
%   \includegraphics[scale = 0.2]{figure/bl_-2.jpg}
%   \label{fig:bl2}
% \end{figure}
\begin{figure}[h!]
\centering
  \includegraphics[width=\linewidth]{figure/bl_8.jpg}
  % \vspace{4cm}
  % \caption{Top left: Probability distribution of the MINI-RGBD's bone length of the bone between right knee and right foot. Top right: Distribution of the same bone in our augmentation data. Bottom Line: Distributions of the bone angle between left should and left elbow. Our augmented data span over a wider range of bone length.}
  \caption{A graph shows the data distribution of bone length in the augmented dataset is better than the original MINI-RGBD. Our augmented dataset spans over a wider range of bone length.}
  \label{fig:bl1}
\end{figure}

% \begin{figure}[h!]
% \centering
%   \includegraphics[scale = 0.2]{figure/bl_-2.jpg}
%   \caption{Left: Probability distribution diagram of the MINI-RGBD's bone length of . Right: Probability distribution diagram of the same bone in our augmentation data. Our augmented data span over a wide range of bone length.}
%   \label{fig:bl2}
% \end{figure}

\begin{figure}[h!]
\centering
  \includegraphics[width=\linewidth]{figure/ba_10.jpg}
  \caption{A graph shows the data distribution of bone angle in the augmented dataset is better than the original MINI-RGBD. Our augmented data have a wider range of bone angles.}
  \label{fig:angle1}
\end{figure}

% \begin{figure}[h!]
% \centering
%   \includegraphics[scale = 0.2]{figure/aug_angle_-1.jpg}
%   \caption{Comparison of the bone angles around left elbow between augmentation data and the original MINI-RGBD data. Our augmented data have a wide range of angles.}
%   \label{fig:angle2}
% \end{figure}

% \begin{figure}[h!]
% \centering
%   \includegraphics[scale = 0.2]{figure/syrip_dist.jpg}
%   \caption{Left side: Data distribution of 3D pose of Syrip Dataset. Right side: Data distribution of the augmentation data for Syrip. As Syrip dataset is extracated from online resources so the data distribution is already full of diversity. In this case, our data augmentation only produces more data for training. }
%   \label{fig:dist_aug}
% \end{figure}



\subsection{Data Augmentation Diversity}
\label{sec:ablation_aug}
In this section, we try to demonstrate in figure \ref{fig:dist_aug} how our condition-guided data augmentation method enhances diversity of the MINI-RGBD dataset. In experiment, we add 4000 augmented data and its distribution is displayed on the right side of the figure. By observation, our method indeed increases more diversity.
To look into pose kinematics in details, we analyze bone lengths and bone angles of the original MINI-RGBD dataset and our augmented data. As shown in figure \ref{fig:bl1}, we choose two bones and compare their bone lengths. Our augmented data bone length spans over a wider range of scale. Similarly, we show comparison results of bone angles in \ref{fig:angle1} and get the same conclusion, which further validates our data augmentation method's enhancement in diversity. 
Table \ref{tab:few_data_mini} and \ref{tab:few_data_syrip} also proves this conclusion quantitatively. 

\subsection{Comparison with 3D pose estimation model}
We want to prove how efficient our two-stage optimization method is, we compare its performance with other classic learning-based 3D pose estimation models widely applied in the human pose estimation area. We trained all the models from scratch on infant datasets without data augmentation and only compare with our plain InfPose. 
\\
In table\ref{tab:compare}, our method still outperforms the other models, which further proves that our previous presumption is correct. We claim that our optimization method fits the task of small-dataset domain adaption 3D pose estimation the most among all these models.  


\begin{table}[t]
\centering
\resizebox{0.6\linewidth}{!}{%
\setlength{\tabcolsep}{0.1cm}
\begin{tabular}{l | c | c }
\toprule
 Datasets   & InfPose  & VideoPose3D\cite{pavllo20193d}\\
\midrule
  SyRIP   &\textbf{49.6} & 145.7\\
  
 
  
  % & Ci \etal\cite{ci2023gfpose}~(S=200)(S=200) & 35.6 & 16.9\\

\bottomrule
\end{tabular}
}
\caption{MPJPE performance of different pose esimation models trained from scratch with no augmentation. Clearly our method is more suitable for the infant small dataset than other learning-based models.}
\label{tab:compare}
% \end{adjustbox}
\end{table}

% \subsection{Optimization Iteration Times}


% \subsection{Diffusion Noise Level}

==> sec/07_conclusion.tex <==
\section{Limitation}
Though our method have impressive capacity in small datasets like infant 3D pose, it still needs accurate 2D keypoints from existing detectors. 
Additionally, the prediction results of our method also depends on the depth distance $T_{o}$ defined in initialization, since we find that the generation model only learns root-relative priors and has little knowledge of spatial depth. 
Besides, like all other optimization works aiming to minimize 2D-3D projection error, our method may also suffer from one-to-many mappings even if this rarely happens. For example, there are 3 outliners in MINI-RGBD. We take an failure example with the highest error in figure \ref{fig:failure}. Though their 2D projects are mapped, our model fails to predict correct $T$ of 3D keypoints. 


\begin{figure}[h!]
\centering
  \includegraphics[width=\linewidth]{figure/failure.jpg}
  \caption{One of the failure examples achieves the highest MPJPE in MINI-RGBD. Left side: our prediction. Right side: ground truth.}
  \label{fig:failure}
\end{figure}


\begin{figure}[h!]
\centering
  \includegraphics[scale=0.3]{figure/mini_vis.pdf}
  \caption{Visualizations of our method on MINI-RGBD. Left: original image. Middle: ground truth 2D pose. Right: Our prediction in red and 3D ground truth in blue are mapped well.}
  \label{fig:mini_vis}
\end{figure}

\begin{figure}[h!]
\centering
  \includegraphics[scale = 0.3]{figure/syrip_vis.pdf}
  \caption{Visualizations of our method on Syrip. Left: original image. Middle: ground truth 2D pose. Right: Our prediction in red and 3D ground truth in blue. The shape and pose in general is well aligned but there's still little gap in depth. Considering that no camera parameter is given, this performance is still acceptable.}
  \label{fig:syrip_vis}
\end{figure}

\section{Conclusion}
In summary, we propose an optimization method which applies a Score Matching Network to the generative priors of infant pose. We show that our method could achieve SOTA on MINI-RGBD and SyRIP, and attain efficient domain adaptation using a small amount of data. We compare three different kinds of adaptation strategies of our model, in which fine-tuning an adult pre-trained generative model seems efficient for MINI-RGBD and the full SyRIP, and the controllable version is also comparable. We also introduce a condition-guided diffusion model as data augmentation trick which enhances diversity and performance for all the three strategies. We fully prove that our method perfectly fits the requirements of small-dataset adaptation work in the realm of 3D infant pose estimation. 

==> sec/background.tex <==
\section{Related Work}




% \subsection{Optimization in Human Pose Estimation}
% Optimization method is good at doing inference case by case and not easily influenced by domain gap and out-of-distribution issue.  Optimization work does not depend on the number of data much for training but requires high accuracy of 2D detection. In the case of small datasets, we believe that an optimization track is more reliable than learning-based models.

\subsection{Adult Human Pose Estimation}
There are mainly two tracks in the human pose estimation area. One-stage method aim to directly predict 3D keypoints or model from raw images, and two-stage ones use 2D  detector to extract 2D keypoints first as an intermediate step and lift 2D to 3D. For instance, 
In~\cite{pavllo20193d}, they apply dilated temporal convolution to enhance 3D pose estimation for unlabeled videos in an semi-supervised method. Zhao \etal~\cite{zhao2019semantic} designs a novel graph convolution and takes advantage of GCN to learn inter-joint features and local and global relationships in a structured graph.  Yang~\etal~\cite{yang2023camerapose} choose to use the 2D annotations in the wild to improve prediction quality, in an weakly supervised method.
Traditionally, one-stage method is more challenging as images may vary to a great extent so it is generally harder to do inference in the wild or cross evaluation. Therefore we follow two-stage track for accuracy as 2D detectors now are fully developed, even in the infant domain~\cite{syrip}.
\\
There are also two tracks inside the 2D-3D lifting networks. Learning-based methods depend on deep-learning models to learn 2D-3D inter-relationships and usually achieve higher accuracy. Researchers thus prefer this track in these days and all the related works we mentioned above fall into this branch. Nevertheless, learning-based models require sufficient data to support training and suffer from generality around datasets in different domain~\cite{chai2023global}. So this strategy is hard to work in small datasets. Other than learning-based models, optimization methods are good at doing inference case by case so they are insusceptible to domain gap and out-of-distribution issues. For example, SMPLify~\cite{bogo2016smplify} uses SMPL~\cite{SMPL} model to do optimization via minimizing kinetic constraints and model to 2D projection error. Furthermore, SMPLift-XMC~\cite{muller2021SMPLify-XMC} takes into account of age and height, and add more advanced constraints on the base of SMPLify. In ~\cite{8486576}, they build a novel video scene system to predict 3D pose, tracklets and actions under overlapping views collected by cameras. In ~\cite{wang2014robust}, they represent a 3D pose as a linear combination of base learned from 3D skeletons and also follow 3D-2D projection constraints and limb length. The advantage of this branch is that these methods do not depend on a large number of training data and they are more general and friendly to domain transfer. Taking all of these factors into account, we finally choose to use a two-stage optimization based method to achieve considerable performace in small datasets.

% \subsection{Diffusion Model in Human Pose Estimation}
% Nowadays, diffusion model becomes one of the most popular topics due to its outstanding capacity of image generation and denoising. As a strong generative model, a lot of previous work have proven that it is a reliable prior learner~\cite{}. In human pose estimation, ~\cite{} applies a GNN-based backbone and a sequence of 2D pose as conditions to predict 3D keypoints. Furthermore, ~\cite{} uses 2D as condition and proposes a new mask strategy to unify denoising, 3D generation and 3D prediction. Though we choose to apply a Score Matching NetWork diffusion model as our generative priors, our model is only trained on 3D pose data without 2D conditions for guidance. Once 2D condition involves in training, the diffusion model may still suffer from out-of-distribution issues. 

\subsection{3D Infant Pose Estimation}
To fully understand and analyze infant behavior in space, 3D infant pose estimation requires high accuracy. A lot of previous work focus on predicting 3d keypoints from RGBD data. Wu~\etal~\cite{wu93} measured infant movements by combining 2D keypoints and matching depth images collected by Kinect. Li~\cite{li2020three} continues using the same pipline but correcting depth information for a better matching between image and depth. However, Kinect may cause depth ambiguity if joints are occluded and depth images are not always available in infant monitor system. In ~\cite{ellershaw3d}, the author uses a 2D pose estimation model and a 3D lifting network pretrained on adult dataset and fine-tuned on infant dataset. Though their model achieve rather good performance on MINI-RGBD dataset, their model are basically learning based and hard to adapt to more realistic data due to domain gap. From our experience in human pose estimation, predicting 3D keypoints from 2D keypoint detection is easier than one-stage method predicting 3D joints from raw images.\\
Moreover, some previous works also apply data augmentation or synthetic data to supplement small datasets. In~\cite{syrip} they collect real data from online resources and also synthesize fake images by augmenting parameters obtained via fitting SMIL~\cite{ma2021smil} model to real infant images. As SMIL has only a few infant textures, they also applied adult appearance as texture. Similarly, in ~\cite{hesse} they also use SMIL model to map infant movements to generate synthetic RGBD images and corresponding 2D 3D keypoint coordinates. However, these methods mainly serve for models which learn image features and generating such images are mostly unnecessary if only keypoints are required. Though we also data augmentation model to help us expand datasets, we don't start from any mesh model but simply add pose in the keypoint space, without explicitly manipulating any parameter.
